Laparoscopic Scene Analysis for Intraoperative Visualisation of Gamma Probe Signals in Minimally Invasive Cancer Surgery

Cancer remains a significant health challenge worldwide, with a new diagnosis occurring every two minutes in the UK. Surgery is one of the main treatment options for cancer. However, surgeons rely on the sense of touch and naked eye with limited use of pre-operative image data to directly guide the excision of cancerous tissues and metastases due to the lack of reliable intraoperative visualisation tools. This leads to increased costs and harm to the patient where the cancer is removed with positive margins, or where other critical structures are unintentionally impacted. There is therefore a pressing need for more reliable and accurate intraoperative visualisation tools for minimally invasive surgery to improve surgical outcomes and enhance patient care. A recent miniaturised cancer detection probe (i.e., SENSEI developed by Lightpoint Medical Ltd.) leverages the cancer-targeting ability of nuclear agents to more accurately identify cancer intra-operatively using the emitted gamma signal. However, the use of this probe presents a visualisation challenge as the probe is non-imaging and is air-gapped from the tissue, making it challenging for the surgeon to locate the probe-sensing area on the tissue surface. Geometrically, the sensing area is defined as the intersection point between the gamma probe axis and the tissue surface in 3D space but projected onto the 2D laparoscopic image. Hence, in this thesis, tool tracking, pose estimation, and segmentation tools were developed first, followed by laparoscope image depth estimation algorithms and 3D reconstruction methods.

==> chapters/chapter1-introduction/3-roadmap.tex <==
\section{Thesis roadmap}

Describe the structure of the thesis - what is in each section and how does the story flow from one to the next.

==> chapters/chapter3-contribution_1-Tracking/3-relatedwork.tex <==
\section{Related Work}
\label{rw_proble_tracking}
\anh{\textbf{TODO: Rewrite}}

\textbf{\anh{need to move and merge this paragraph to the intro} }Minimally invasive surgery (MIS) is becoming a standard procedure for a range of surgical disciplines. Advantages of MIS include less blood loss, less post-operative pain, lower infection rates and shorter hospitalisation. However, there are intrinsic limitations to existing MIS approaches, including a loss of direct organ manipulation, lack of dexterity via ‘keyhole’ access and poor depth perception using a monocular laparoscope. To identify anatomical structures such as vessels and tumours, intraoperative ultrasound has been used~\cite{hughes2013intraoperative}. However, a well-known drawback of using intraoperative ultrasound is that surgeons need to interpret the ultrasound images and perceptually relate these images to the operative scene captured by a laparoscope~\cite{mohareri2015intraoperative}. This is particularly challenging, as the ultrasound images and laparoscopic videos are displayed separately on different screens. To reduce the mental workload of a surgeon, a previous study presented in~\cite{hughes2013intraoperative} has introduced an intuitive visualisation method, which is achieved by registering the 2D ultrasound images into the surgical scene. This approach enables surgeons to observe details from both ultrasound and laparoscope in a single diplay. To provide consistent image overlays, the ultrasound probe needs to be tracked during operation. 

A direct use of laparoscopic images for tracking instrument in MIS is more practical than of other methods where extra tracking devices~\cite{feuerstein2007magneto} are used. The introduction of additional tracking devices into the theatre would not only occupy valuable space in the operating field, but also suffer from intrinsic limitations of these tracking devices such as ferromagnetic interference and line-of-sight issues. Previous methods have extracted 2D locations of a planar~\cite{pratt2015robust} or cylindrical~\cite{jayarathne2013robust} marker that is rigidly attached to the probe. In Table~\ref{tab:trackingproble_comparison}, a list of marker-based tracking methods for intraoperative ultrasound probes is presented. %Among these methods, pose estimation is treated as a Perspective-n-Point (PnP) problem [7]. However, pose estimation of a planar marker may provide two ambiguous solutions where the incorrect one should be eliminated [8].



\begin{table}[t]
 \scriptsize
\caption{Visual marker-based tracking methods comparison for intraoperative \textbf{\anh{ultrasound??? or gama}} probe.}
\vspace{-2ex}
\def\arraystretch{1.1}
\begin{center}
\begin{tabular}{l l l l c c c c c }
\toprule
\multicolumn{0}{c}{Method} & \multicolumn{0}{c}{Probe Shape} & \multicolumn{0}{c}{Pattern Type} & \multicolumn{0}{c}{Robotic/freehand} & \multicolumn{0}{c}{AR/VR} & \multicolumn{0}{c}{Real-time} & \multicolumn{0}{c}{Open-source}  \\
\midrule
Pratt~\etal~\cite{pratt2012intraoperative}         & Planar & Chessboard                                       & Freehand  & \anh{???}  & Yes & \anh{???}     \\
Edgcumbe~\etal~\cite{edgcumbe2013calibration} & Planar        & Circular dot  & Robotic & \anh{???}  & No        & \anh{???}      \\
Pratt~\etal~\cite{pratt2015robust}                   & Planar        & Chessboard  & Robotic & \anh{???}  & Yes        & \anh{???}    \\
Jayarathne~\etal~\cite{jayarathne2013robust}            & Cylindrical        & Chessboard & Freehand & \anh{???}  & No        & \anh{???}     \\
Lin Zhang~\etal~\cite{zhang2017real}          & Cylindrical       & Hybrid & Both & \anh{???}      & Yes & \anh{???}     \\
%You~\etal~\cite{}                & Unity Physics & Discretized                                       & \xmark  & \xmark & Vision-Based & \xmark  \\    
\cmidrule{1-7}
\textbf{Huang}~\etal                          & \anh{???}                & Hybrid  & \anh{???} & Yes & Yes   & \anh{???} \\
\bottomrule
\end{tabular}
\label{tab:trackingproble_comparison}
\end{center}
\end{table}
%\vspace{-1ex}




==> chapters/chapter3-contribution_1-Tracking/3-tables/3-4-example_table.tex <==
\begin{table}[h!]
  \mycaption{Caption Title goes here (appears in TOC).}{Rest of the caption goes here \label{tab:example_table}}
  \centering
  \colorbox{white}{
      \begin{tabular}{ccccc}
      \hline 
      \textbf{Experiment}  		& \textbf{Dataset} 				& \textbf{Size} 		& \textbf{GT} 		& \textbf{Seg. Method} 	\\	\hline		
      A 		& Hammersmith   & 100		& \cmark		& RF 			\\
      B 		& UKBB-2964	    & 4,805		& \cmark		& RF and CNN  	\\
      C 		& UKBB-18545	& 7,250		& \xmark		& Multi-Atlas	\\   \hline
      \end{tabular}
  }%colorbox
\end{table}


==> chapters/chapter3-contribution_1-Tracking/3-tables/3-5-example_results.tex <==
\begin{table}[h]
    \centering
    \mycaption{Table Title (appears in TOC)}{The rest of the caption goes here. \label{tab:3-example_results}}
    \colorbox{white}{
    \begin{minipage}[t]{0.5\linewidth}
        \begin{tabular}[t]{r | c c c c}
            \textbf{Class}	&   \textbf{Metric}  &    \textbf{Acc}.	&	\textbf{TPR}	&	\textbf{FPR}	\\
            \hline							
            \textbf{LVC}	&	DSC	&	0.998	&	1.000	&	0.000	\\
            	&	MSD	&	1.000	&	1.000	&	0.000	\\
            \textbf{LVM}	&	DSC	&	0.051	&	1.000	&	0.001	\\
            	&	MSD	&	1.000	&	1.000	&	0.000	\\
            \textbf{RVC}	&	DSC	&	0.901	&	1.000	&	0.033	\\
            	&	MSD	&	0.997	&	0.997	&	0.000	\\
            \textbf{Av.}	&	DSC	&	0.650	&	1.000	&	0.011	\\
            	&	MSD	&	0.999	&	0.999	&	0.000	\\
            \textbf{WH}	&	DSC	&	\textbf{0.998}	& \textbf{1.000}	&	\textbf{0.000}	\\
            	&	MSD	&	\textbf{1.000}	&	\textbf{1.000}	&	\textbf{0.000}	\\
        \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.45\linewidth}
        \begin{tabular}[t]{r | c c c c}
            & \multicolumn{4}{c}{\textbf{MAE}} \\
            \hline
            \thead{\textbf{Class}} & \thead{\textbf{DSC}\\} & \thead{\shortstack{\textbf{MSD}\\(mm)}} & \thead{\shortstack{\textbf{RMS}\\(mm)}} & \thead{\shortstack{\textbf{HD}\\(mm)}}\\
            \hline									
            \textbf{LVC}	&	0.082	&	0.386	&	0.442	&	1.344	\\
            \textbf{LVM}	&	0.268	&	0.510	&	0.547	&	2.127	\\
            \textbf{RVC}	&	0.146	&	0.588	&	0.656	&	2.086	\\
            \textbf{Av.}	&	0.165	&	0.495	&	0.548	&	1.852	\\
            \textbf{WH}	&	\textbf{0.089}	&	\textbf{0.460}	&	\textbf{0.509}	&	\textbf{1.698}	\\
        \end{tabular}
    \end{minipage}
    }%colorbox
\end{table}

==> chapters/chapter6-conclusions/6-further_work.tex <==
\section{Further Work}
\label{sec:6-further_work}
\glsresetall

Outline of the future work to be done in this area. What are the immediate next steps for this line of research? What would be done further down the line? Which areas are interesting to explore? What has changed since this work was done?

If using this template, you should also attribute the formatting to Rob Robinson \parencite{robinson2020thesis} and link to the original template or thesis \url{https://github.com/mlnotebook}.


==> chapters/chapter6-conclusions/6-limitations.tex <==
\section{Limitations}
\label{sec:6-limitations}
\glsresetall

The primary limitations are laid out here and then discussed afterwards.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\colorlet{shadecolor}{Sepia!5}
\begin{shaded*}
\textbf{Chapter 1 Title}
    \begin{enumerate}[wide, leftmargin=0.75cm, labelwidth=!, labelindent=0pt, label=\textbf{\Alph*}]
    \singlespacing
    \item Limitation 1.
    \item Limitation 2.
    \item Limitation 3.
    \end{enumerate}
\end{shaded*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\colorlet{shadecolor}{Sepia!5}
\begin{shaded*}
\textbf{Chapter 2 Title}
    \begin{enumerate}[wide, leftmargin=0.75cm, labelwidth=!, labelindent=0pt, label=\textbf{\Alph*}]
    \singlespacing
    \item Limitation 1.
    \item Limitation 2.
    \item Limitation 3.
    \end{enumerate}
\end{shaded*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\colorlet{shadecolor}{Sepia!5}
\begin{shaded*}
\textbf{Chapter 3 Title}
    \begin{enumerate}[wide, leftmargin=0.75cm, labelwidth=!, labelindent=0pt, label=\textbf{\Alph*}]
    \singlespacing
    \item Limitation 1.
    \item Limitation 2.
    \item Limitation 3.
    \end{enumerate}
\end{shaded*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Chapter 1 Limitations}

Explanation of the limitations gathered from Chapter 1 and potential approaches for overcoming them.

\subsection{Chapter 2 Limitations}

Explanation of the limitations gathered from Chapter 2 and potential approaches for overcoming them.

\subsection{Chapter 3 Limitations}

Explanation of the limitations gathered from Chapter 3 and potential approaches for overcoming them.


==> chapters/chapter6-conclusions/6-main_conclusions.tex <==
\section{Main Conclusions}
\label{sec:6-main_conclusions}
\glsresetall

A brief summary of the ideas that this Thesis has explored. The main contributions are then laid out in summary below then discussed further afterwards.

If using this template, you should also attribute the formatting to Rob Robinson \parencite{robinson2020thesis} and link to the original template or thesis \url{https://github.com/mlnotebook}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\colorlet{shadecolor}{MidnightBlue!5}
\begin{shaded*}
\textbf{Chapter 1 Title}
    \begin{enumerate}[wide, leftmargin=0.75cm, labelwidth=!, labelindent=0pt, label=\textbf{\Alph*}]
    \singlespacing
    \item Conclusion 1.
    \item Conclusion 2.
    \item Conclusion 3.
    \end{enumerate}
\end{shaded*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\colorlet{shadecolor}{MidnightBlue!5}
\begin{shaded*}
\textbf{Chapter 2 Title}
    \begin{enumerate}[wide, leftmargin=0.75cm, labelwidth=!, labelindent=0pt, label=\textbf{\Alph*}]
    \singlespacing
    \item Conclusion 1.
    \item Conclusion 2.
    \item Conclusion 3.
    \end{enumerate}
\end{shaded*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\colorlet{shadecolor}{MidnightBlue!5}
\begin{shaded*}
\textbf{Chapter 3 Title}
    \begin{enumerate}[wide, leftmargin=0.75cm, labelwidth=!, labelindent=0pt, label=\textbf{\Alph*}]
    \singlespacing
    \item Conclusion 1.
    \item Conclusion 2.
    \item Conclusion 3.
    \end{enumerate}
\end{shaded*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Chapter 1 Conclusions}

Explanation of the conclusions gathered from Chapter 1 and how they fit into the overall idea of the Thesis.

\subsection{Chapter 2 Conclusions}

Explanation of the conclusions gathered from Chapter 2 and how they fit into the overall idea of the Thesis.

\subsection{Chapter 3 Conclusions}

Explanation of the conclusions gathered from Chapter 3 and how they fit into the overall idea of the Thesis.

==> meta/chapterheads.tex <==
%%%%% Chapter Headings %%%%%%
% NUMBERED CHAPTED HEADING
\makeatletter
\def\thickhrule{\leavevmode \leaders \hrule height 0.25ex \hfill \kern \z@}
\def\position{\centering}
\renewcommand{\@makechapterhead}[1]{%
  \vspace*{2\p@}%
  {\vfill\parindent \z@
        {  \vfill\raggedright\LARGE {\fontsize{20pt}{20pt}\selectfont Chapter \thechapter} }
        \par\nobreak
        {\thickhrule}
        \vspace*{1\p@}%
        \interlinepenalty\@M
        \par\nobreak
        \vspace*{1\p@}%
        {\raggedright\bfseries\fontsize{26pt}{26pt}\selectfont {#1}\par\nobreak}
        \par\nobreak
        \vspace*{1\p@}}%
    \vskip 10\p@
  }

% STARRED CHAPTER HEADING (e.g. Preamble Dedication, Acknowledgements...)
\def\@makeschapterhead#1{%
  \vspace*{2\p@}%
  {\parindent \z@
        {\thickhrule}
        \par\nobreak
        \vspace*{1\p@}%
        \interlinepenalty\@M
        \par\nobreak
        \vspace*{1\p@}%
        {\raggedright\bfseries\fontsize{26pt}{26pt}\selectfont {#1}\par\nobreak}
        \par\nobreak
        \vspace*{1\p@}%
    \vskip 10\p@}
  }
\makeatother

\setlength{\headheight}{14.5pt}

==> meta/code.tex <==
\usepackage[newfloat]{minted}
\renewcommand*{\listlistingname}{List of Source Code}

\newenvironment{longlisting}{\captionsetup{type=listing,justification=raggedright,singlelinecheck=false}}{}

\setminted[python]{
linenos,
firstline=9,
baselinestretch=0.8,
frame=single,
bgcolor=black!2,
breaklines=true,
firstnumber=1,
tabsize=3,
fontfamily=tt,
fontsize=\fontsize{9pt}{11pt}\selectfont,
baselinestretch=1}

\usemintedstyle{vs}

==> postamble/appendices/2-code/code_listing.tex <==
\clearpage

==> preamble/acknowledgements.tex <==
\clearpage
\chapter*{Acknowledgements}

My heart brims with gratitude and admiration for my esteemed advisor, Daniel Elson. His decision to mentor me during my PhD studies was a true blessing, granting me the gift of a lifetime: the opportunity to surpass mediocrity, sharpen my intellect through scholarly research, and cultivate the self-assurance to stand tall in the world. Throughout my academic journey, Dan's unwavering support came in many forms, from patiently teaching me LabVIEW to steering me towards cutting-edge research and encouraging me to validate our findings in the operating theater. Applying our research to clinical practice was a daunting and costly task, but an essential one that would ultimately benefit society. As I move forward in my career, I will carry Dan's belief and carefree mindset with me, always striving to uphold his courage and honor the invaluable lessons he imparted upon me. %His influence on my life has been immeasurable, and I will forever be indebted to him for the countless ways in which he has supported and inspired me.


I also want to express my sincere thanks to my second supervisor, Stamatia Giannarou, for her immeasurable influence and patient guidance during my doctoral studies. She exuded an unparalleled passion for research and was always considerate towards her students, putting their best interests at heart. %and I feel blessed to have had her as my mentor. 
During my PhD, she provided me with opportunities to co-chair Hamlyn Symposium, which allowed me to develop my organizational and interpersonal skills. Her invaluable support and encouragement have been a source of strength and comfort for me. I am forever grateful for her kindness and will never forget the piece of chocolate cake from her on the day when I was at my lowest point.

I am overflowing with gratitude towards my co-author, Anh Nguyen, whose companionship and support have been an indispensable source of strength throughout this journey. From the moment I was first introduced to deep learning, Anh %stood by my side, offering constant encouragement and boundless inspiration. He 
has always been willing to lend an ear to my research progress and ideas, and his keen insights and suggestions have proven to be instrumental to my success. Anh's dedication to excellence and
comprehensive knowledge of research have been remarkable and impressive, serving as a shining example for me to emulate. I will forever cherish our collaboration, and I am proud to have worked alongside such an exceptional researcher and friend. 

It is with great pleasure for me to say thanks to the National Institute for Health Research (NIHR) for sponsoring the research project, and to Lightpoint Medical Ltd., for their generous support throughout our collaboration. As the Lightpoint Medical Ltd. is currently being acquired and I am completing my PhD, I am grateful for the success of this project, which was made possible by their contributions. I am also thankful for the Hamlyn Center team, which is a friendly and innovative group of individuals. I have found kindred spirits here, with the camaraderie and support of my senior colleagues and peers. I am particularly grateful for their trust in my abilities and their guidance, which have helped me grow both personally and professionally.


I would like to express my deepest gratitude to my parents, who have given me the opportunity to see the world and supported me endlessly and unconditionally throughout my growth. Their parenting style has enabled me to be resilient and impervious to society's praise or criticism and has given me the confidence and backbone to follow my dreams, pursue what I love, and let go of anything that holds me back. %My father has always encouraged me to go anywhere in the world that brings me happiness and to do anything that brings me joy, without worrying about my family or any other constraints. He has always wished for me to live a carefree life with the courage to follow my dreams. My mother, on the other hand, has always believed in my ability to change the world. She has encouraged me to climb the highest mountains, explore the farthest corners of the earth, experience success and failure, meet people from all walks of life, and eventually make a name for myself in my chosen field. Their parenting style has enabled me to be resilient and impervious to society's praise or criticism and has given me the confidence to say no to any temptation. Their unwavering support has given me the backbone to pursue what I love and let go of anything that holds me back.



%I want to express my gratitude to my past self, who never gave up and kept moving forward. I am thankful for my unwavering determination in the face of uncertainty, for my courage in the midst of setbacks and hardships, and for my readiness to confront various challenges. I appreciate my past self's proactive preparation for every opportunity that came my way. Starting from now and for a long time to come, I will cherish the memories of my doctoral studies. Those were the brightest and most carefree moments of my life, and I will always look back upon them with fondness.

%Starting from this very moment and for every day to come, I will hold dear the memories of my doctoral studies as the most brilliant and carefree moments of my life. These precious moments will forever be etched in my heart, and I will always look back upon them with a sense of joy and gratitude. I am thankful for the opportunities and experiences that have shaped me into the person I am today, and I will carry them with me always, wherever my journey takes me.

Starting from this time and for every day to come, I will hold dear the memories of my doctoral studies as the most brilliant and carefree moments of my life. I am thankful for the opportunities and experiences that have shaped me into the person I am today. These precious time will forever be etched in my heart. I will always look back upon them with a sense of joy and gratitude, and I will carry them with me always, wherever my journey takes me.
